Parallel Calibration for Sensor Array Radio Interferometers

In order to meet the theoretically achievable imaging performance, calibration of modern radio interferometers is a mandatory challenge, especially at low frequencies. In this perspective, we propose a novel parallel iterative multi-wavelength calibration algorithm. The proposed algorithm estimates the apparent directions of the calibration sources, the directional and undirectional complex gains of the array elements and their noise powers, with a reasonable computational complexity. Furthermore, the algorithm takes into account the specific variation of the aforementioned parameter values across wavelength. Realistic numerical simulations reveal that the proposed scheme outperforms the mono-wavelength calibration scheme and approaches the derived constrained Cram\'er-Rao bound even with the presence of non-calibration sources at unknown directions, in a computationally efficient manner.

==> preambule.tex <==
%------------------------------------
% Packages initiaux (à placer au début)
%------------------------------------

 \usepackage[utf8x]{inputenc}
 \usepackage[T1]{fontenc}
 \usepackage[english]{babel}
 \usepackage[english]{varioref}
 \usepackage[left=2cm,right=2cm,top=2cm,bottom=2cm, headheight=15 pt]{geometry}
 \usepackage{etex} % Package pour augmenter la mémoire
%  \usepackage{cmbright}
%    \usepackage{beton, euler}
 \usepackage{kpfonts}

% %------------------------------------
% % % Police d'écriture
% %------------------------------------
% 
\usepackage{siunitx} % Package unité
\sisetup{detect-all = true}
\usepackage[dvipsnames]{xcolor}
\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\definecolor{mymauve}{rgb}{0.58,0,0.82}
%\usepackage{wasysym} % Pour les smileys et autres symboles
%------------------------------------
% Packages de mise en page / formatage
%------------------------------------
%\usepackage{ccaption} % Modification des légendes
\usepackage{enumitem} % Modification des listes à puces
\usepackage{pifont} % Modification des listes à puces
% ---------
% Entêtes
% ---------
\usepackage{lastpage} % Connaître le numéro de la dernière page
\usepackage{fancyhdr}
\pagestyle{fancy}

%------------------------------------
%FORMAT DES SECTIONS, SOUS-SECTIONS,...
%------------------------------------
\usepackage{titlesec}
\definecolor{bleu_ens}{RGB}{0,72,153}
\newcommand{\HRule}{{\color{bleu_ens}\rule{\linewidth}{1mm}}}
\renewcommand{\chaptertitlename}{Part}
\renewcommand{\thechapter}{\Roman{chapter}}
\renewcommand{\thesubsection}{\arabic{subsection}}
\newcounter{mysubsubsection}[subsection]
\renewcommand{\thesubsubsection}{\alph{mysubsubsection}}
\setcounter{secnumdepth}{3}
\titleformat{\chapter}[display]{\huge\bfseries}
{\LARGE\filleft\MakeUppercase{\chaptertitlename} \thechapter}{4ex}{\titlerule\vspace{2ex}\filright}[\vspace{2ex}\titlerule]

\titleformat{\section}{\LARGE\fontfamily\bfseries}{\thesection}{1em}{}
\titlespacing{\section}{0pc}{4.5ex plus .1ex minus .2ex}{2.5ex minus .1ex}

\titleformat{\subsection}{\LARGE\sffamily\slshape}{\thesubsection}{1em}{}
\titlespacing{\subsection}{1pc}{3.5ex plus .1ex minus .2ex}{1.5ex minus .1ex}

\titleformat{\subsubsection}{\Large\fontfamily\slshape}{}{1em}{}%\stepcounter{mysubsubsection}\thesubsubsection)~
\titlespacing{\subsubsection}{2pc}{3.0ex plus .1ex minus .2ex}{1.0ex minus .1ex}
\assignpagestyle{\chapter}{fancy}


\usepackage{setspace}

%------------------------------------
%Insertion d'images
%------------------------------------
\usepackage{graphicx}
%\usepackage{subcaption}

%\usepackage{multicol}
%\usepackage{subfiles}
\usepackage[
	colorlinks=false, 
	urlcolor=red, 
	breaklinks, 
	%pagebackref, 
	citebordercolor={0 0 0}, 
	filebordercolor={0 0 0}, 
	linkbordercolor={0 0 0}, 
	runbordercolor={0 0 0}, 
	urlbordercolor={0 0 0}, 
	pdfborder={0 0 0},
	pdfauthor = {Martin BROSSARD}
	]{hyperref} 
%\usepackage{makeidx}
\usepackage{changepage}
\usepackage{wrapfig}

\usepackage{listings}
\lstset{ %
  backgroundcolor=\color{white},   
  basicstyle=\footnotesize,        
  breakatwhitespace=false,         
  breaklines=true,                 
  captionpos=b,                   
  commentstyle=\color{mygreen},    
  deletekeywords={...},            
  escapeinside={\%*}{*)},          
  extendedchars=true,              
  frame=single,               
  keepspaces=true,                 
  keywordstyle=\color{blue},       
  morekeywords={*,...},            
  numbers=right,                   
  numbersep=10pt,                   
  numberstyle=\tiny\color{mygray}, 
  rulecolor=\color{black},         
  showspaces=false,                
  showstringspaces=false,          
  showtabs=false,                  
  stepnumber=5,                    
  stringstyle=\color{mymauve},     
  tabsize=4,                       
  title=\lstname,
  literate=%
         {à}{{\`a}}1
         {í}{{\'i}}1
         {é}{{\'e}}1
         {è}{{\`e}}1
         {ê}{{\^e}}1
         {ý}{{\'y}}1
         {ú}{{\'u}}1
         {ù}{{\`u}}1
         {ó}{{\'o}}1
         {ç}{{\c{c}}}1
         {ě}{{\v{e}}}1
         {š}{{\v{s}}}1
         {č}{{\v{c}}}1
         {ř}{{\v{r}}}1
         {ž}{{\v{z}}}1
         {ď}{{\v{d}}}1
         {ť}{{\v{t}}}1
         {ň}{{\v{n}}}1                
         {ů}{{\r{u}}}1
         {Á}{{\'A}}1
         {Í}{{\'I}}1
         {É}{{\'E}}1
         {Ý}{{\'Y}}1
         {Ú}{{\'U}}1
         {Ó}{{\'O}}1
         {Ě}{{\v{E}}}1
         {Š}{{\v{S}}}1
         {Č}{{\v{C}}}1
         {Ř}{{\v{R}}}1
         {Ž}{{\v{Z}}}1
         {Ď}{{\v{D}}}1
         {Ť}{{\v{T}}}1
         {Ň}{{\v{N}}}1                
         {Ů}{{\r{U}}}1                  
}

%---------------------------------------
% Packages scientifiques/mathématiques
%---------------------------------------
%
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{bm}
% %\usepackage{mathenv}
% %\usepackage{array}
% 
\usepackage[english, onelanguage,ruled,vlined, algochapter, longend]{algorithm2e} % package pseudo-algorithme , boxed
\SetAlgoSkip{Bigskip} 


%---------------------------------------
% Packages graphique
%---------------------------------------

\usepackage{pgfplots}
\usepackage{tikz}
\usetikzlibrary[patterns]
\pgfplotsset{compat=1.12}
\usepackage[final]{pdfpages}


\usepackage{caption}
\captionsetup{justification=centering,labelfont={bf},font={normal,it},width=0.75\textwidth}

%---------------------------------------
% Opérateurs mathématiques
%---------------------------------------

%---------------------------------------
% En-tête et pied de page
%---------------------------------------
\usepackage{fancyhdr}
\pagestyle{fancy}

\renewcommand{\headrulewidth}{1pt}
\renewcommand{\footrulewidth}{1pt}
\fancyhead[L]{}
\fancyhead[C]{}
\fancyhead[R]{}
\fancyfoot[L]{}
\fancyfoot[C]{}
\fancyfoot[R]{\thepage /\pageref{LastPage}}
%---------------------------------------
% Environnements
%---------------------------------------

%Renommage des figuges et des tableaux
%\addto\captionsfrench{\def\figurename{}}
%\addto\captionsfrench{\def\tablename{}}

%---------------------------------------
% Commandes perso
%---------------------------------------
\newcommand{\eg}{\emph{e.g.} }
\newcommand{\ie}{\emph{i.e. }}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
%---------------------------------------
% Poubelle
%---------------------------------------
%\usepackage{schemabloc}
%\usepackage{pgfplots}
%\usepackage{chemist}
%\usepackage{setspace}
%\usepackage{chngpage}
%\setlength{\parskip}{0.5ex minus .1ex}
%\usepackage{hhline}
%\usepackage{float}
%\usepackage{subfig}
%\setcounter{secnumdepth}{3}
%\usepackage{fancyvrb}
%\usepackage{perpage} 
%\MakePerPage{footnote}
%\usepackage{array}
%\usepackage{moreverb}
% \usepackage{multirow}
% \usepackage{arydshln}
% \usepackage{float}
\usepackage[space]{cite}
% \usepackage[bottom]{footmisc}
